Lepton Number Violation from Colored States at the LHC

The possibility to search for lepton number violating signals at the Large Hadron Collider (LHC) in the colored seesaw scenario is investigated. In this context the fields that generate neutrino masses at the one-loop level are scalar and Majorana fermionic color-octets of SU(3). Due to the QCD strong interaction these states may be produced at the LHC with a favorable rate. We study the production mechanisms and decays relevant to search for lepton number violation signals in the channels with same-sign dileptons. In the simplest case when the two fermionic color-octets are degenerate in mass, one could use their decays to distinguish between the neutrino spectra. We find that for fermionic octets with mass up to about 1 TeV the number of same-sign dilepton events is larger than the standard model background indicating a promising signal for new physics.

==> Section_mu2egamma.tex <==


\subsection{Constraints from Lepton Flavour Violation: $\mu \to e \gamma$}
Neutrino oscillations indicate the presence of lepton flavor violating operators which lead to various rare decays, the most stringily constrained being $\mu \to e \gamma$.  The colored seesaw  has a contribution which can potentially disagree with experiments (see Fig. \ref{mu2egamma}).

\includegraphics{FeynDiags_Sept01/mu2egamma.pdf}

The branching ratio for this process is given by \footnote{Note: our results agrees with \cite{Liao:2009fm} up to the normalization for the Yukawa couplings, but not with \cite{Losada:2009yy}.}

\begin{equation}
	\text{Br}\left(\mu \to e \gamma \right)
		= \frac{3 \, \alpha_{EM}}{4 \, \pi \, m_S^4 \, G_F^2}
		\left|
			\displaystyle\sum_{\alpha=1}^{2} Y_\nu^{1\alpha} Y_\nu^{\alpha 2 *} F_2\left(x_\alpha\right)
		\right|^2
\end{equation}
where
\begin{align}
x_\alpha & = \frac{m_{F_\alpha}^2}{m_S^2}
\\
F_2\left(x\right) & = \frac{1 - 6 \, x + 3 \, x^2 + 2 \, x^3 - 6 \, x^2 \, \ln x}{12 \left(x-1\right)^4}
\end{align}
It is clear from the above that this branching ratio is very sensitive to the Yukawa couplings: $\text{Br}\left(\mu \to e \gamma \right) \sim Y_\nu^4$.  Only for order one Yukawa couplings does this process conflict with the experimental bound of $\text{Br}\left(\mu \to e \gamma \right) < 10^{-11}$, which will improve by two orders of magnitude at J-Park.  This corresponds to $\lambda \sim 10^{-10}$ for the quartic coupling between the octet scalar and the SM Higgs.  While one can claim that this is inline with the spirit of the seesaw mechanism (order one Yukawa couplings) there is no argument for why this coupling should be so small, although its value is protected by global $U(1)$ lepton number.  Nevertheless, the interplay of the low energy constrains with the collider signatures can be exciting in this part of the parameter space.  For concreteness, we analyze $\lambda = 10^{-11}$ in the normal hierarchy where the Yukawas are order one and for the tri-bimaximal mixing Ansatz $\text{Br}\left(\mu \to e \gamma \right) = 4 10^{-8}$; a value that is already ruled out.  For degenerate $F_1$ and $F_2$, the branching ratio is sensitive only to the neutrino parameters and not to $\omega$, with the greatest sensitivity due to $\sin_{13}$ and for $\sin_{13} \sim -0.09$, the branching ratio can be made arbitrarily small.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}
%\begin{center}
%		\begin{picture}(288,180)
%			\put(0,0){\includegraphics[scale=1]{imgBrVomega}}
%		\end{picture}
%\end{center}
%	\caption
%	{
%		Branching ratios versus omega for values of $s_{13}$ that make $\text{Br}\left(\mu \to e
%		\gamma \right)$ arbitrarily small ($s_{13} \sim -0.09$), with $m_S = 1000$ GeV, $m_{F_1} =
%		m_{F_2} = 1200$ GeV, tri-bimaximal values for the other angles, zero phases and central values
%		for the neutrino masses.
%	}
%	\label{BrVomegas13}
%\end{figure}



